GeoFormer: Learning Point Cloud Completion with Tri-Plane Integrated Transformer

Point cloud completion aims to recover accurate global geometry and preserve fine-grained local details from partial point clouds. Conventional methods typically predict unseen points directly from 3D point cloud coordinates or use self-projected multi-view depth maps to ease this task. However, these gray-scale depth maps cannot reach multi-view consistency, consequently restricting the performance. In this paper, we introduce a GeoFormer that simultaneously enhances the global geometric structure of the points and improves the local details. Specifically, we design a CCM Feature Enhanced Point Generator to integrate image features from multi-view consistent canonical coordinate maps (CCMs) and align them with pure point features, thereby enhancing the global geometry feature. Additionally, we employ the Multi-scale Geometry-aware Upsampler module to progressively enhance local details. This is achieved through cross attention between the multi-scale features extracted from the partial input and the features derived from previously estimated points. Extensive experiments on the PCN, ShapeNet-55/34, and KITTI benchmarks demonstrate that our GeoFormer outperforms recent methods, achieving the state-of-the-art performance. Our code is available at \href{https://github.com/Jinpeng-Yu/GeoFormer}{https://github.com/Jinpeng-Yu/GeoFormer}.

==> figures/result-pcn-2.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/result-pcn-2.pdf}
    % \captionsetup{belowskip=-0.6cm}
    \caption{Visualization comparisons on PCN dataset. Results clearly show that our method can preserve better global structure, and reconstruct better local details.}
    \label{fig:result-pcn-2}
\end{figure}

==> tables/result-sp21-complete.tex <==
% shapenet21 more
\begin{table*}[ht]
	\centering
	% \small
    % \normalsize
	% \scriptsize
	% \setlength{\tabcolsep}{4.5pt}
	\setlength{\arrayrulewidth}{0.7pt}
	\caption{Detailed results for novel 21 categories on ShapeNet-34 dataset. $S.$, $M.$ and $H.$ stand for the simple, moderate and hard difficulty levels.}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
		\toprule[1pt]
		& \multicolumn{3}{c|}{PCN~\cite{yuan2018pcn}} & \multicolumn{3}{c|}{GRNet~\cite{xie2020grnet}} & \multicolumn{3}{c|}{PoinTr~\cite{yu2021pointr}} & \multicolumn{3}{c}{SeedFormer~\cite{zhou2022seedformer}} &
        \multicolumn{3}{c}{Ours}\\
		& S. & M. & H. & S. & M. & H. & S. & M. & H. & S. & M. & H. & S. & M. & H. \\
		\midrule[0.3pt]
		bag			& 2.48 & 2.46 & 3.94 & 1.47 & 1.88 & 3.45 & 0.96 & 1.34 & 2.08 & 0.49 & 0.82 & 1.45 & \textbf{0.43} & \textbf{0.70} & \textbf{1.28} \\
		basket		& 2.79 & 2.51 & 4.78 & 1.78 & 1.94 & 4.18 & 1.04 & 1.40 & 2.90 & 0.60 & 0.85 & 1.98 & \textbf{0.54} & \textbf{0.74} & \textbf{1.66} \\
		birdhouse	& 3.53 & 3.47 & 5.31 & 1.89 & 2.34 & 5.16 & 1.22 & 1.79 & 3.45 & 0.72 & 1.19 & 2.31 & \textbf{0.62} & \textbf{1.01} & \textbf{1.93} \\
		bowl		& 2.66 & 2.35 & 3.97 & 1.77 & 1.97 & 3.90 & 1.05 & 1.32 & 2.40 & 0.60 & 0.77 & 1.50 & \textbf{0.49} & \textbf{0.62} & \textbf{1.10} \\
		camera		& 4.84 & 5.30 & 8.03 & 2.31 & 3.38 & 7.20 & 1.63 & 2.67 & 4.97 & 0.89 & 1.77 & 3.75 & \textbf{0.82} & \textbf{1.63} & \textbf{3.48} \\
		can			& 1.95 & 1.89 & 5.21 & 1.53 & 1.80 & 3.08 & 0.80 & 1.17 & 2.85 & 0.56 & 0.89 & 1.57 & \textbf{0.47} & \textbf{0.72} & \textbf{1.42} \\
		cap			& 7.21 & 7.14 & 10.94 & 3.29 & 4.87 & 13.02 & 1.40 & 2.74 & 8.35 & \textbf{0.50} & 1.34 & 5.19 & 0.57 & \textbf{1.29} & \textbf{3.99} \\
		keyboard	& 1.07 & 1.00 & 1.23 & 0.73 & 0.77 & 1.11 & 0.43 & 0.45 & 0.63 & 0.32 & 0.41 & 0.60 & \textbf{0.28} & \textbf{0.35} & \textbf{0.46} \\
		dishwasher	& 2.45 & 2.09 & 3.53 & 1.79 & 1.70 & 3.27 & 0.93 & 1.05 & 2.04 & 0.63 & 0.78 & 1.44 & \textbf{0.53} & \textbf{0.65} & \textbf{1.15} \\
		earphone	& 7.88 & 6.59 & 16.53 & 4.29 & 4.16 & 10.30 & 2.03 & 5.10 & 10.69 & \textbf{1.18} & 2.78 & \textbf{6.71} & 1.29 & \textbf{2.69} & 7.41 \\
		helmet		& 6.15 & 6.41 & 9.16 & 3.06 & 4.38 & 10.27 & 1.86 & 3.30 & 6.96 & 1.10 & \textbf{2.27} & \textbf{4.78} & \textbf{1.07} & 2.39 & 5.09 \\
		mailbox		& 2.74 & 2.68 & 4.31 & 1.52 & 1.90 & 4.33 & 1.03 & 1.47 & 3.34 & 0.56 & 0.99 & 2.06 & \textbf{0.43} & \textbf{0.88} & \textbf{1.87} \\
		microphone	& 4.36 & 4.65 & 8.46 & 2.29 & 3.23 & 8.41 & 1.25 & 2.27 & 5.47 & 0.80 & \textbf{1.61} & 4.21 & \textbf{0.79} & 1.96 & \textbf{4.20} \\
		microwaves	& 2.59 & 2.35 & 4.47 & 1.74 & 1.81 & 3.82 & 1.01 & 1.18 & 2.14 & 0.64 & 0.83 & 1.69 & \textbf{0.56} & \textbf{0.69} & \textbf{1.36} \\
		pillow		& 2.09 & 2.16 & 3.54 & 1.43 & 1.69 & 3.43 & 0.92 & 1.24 & 2.39 & 0.43 & 0.66 & 1.45 & \textbf{0.37} & \textbf{0.57} & \textbf{1.16} \\
		printer		& 3.28 & 3.60 & 5.56 & 1.82 & 2.41 & 5.09 & 1.18 & 1.76 & 3.10 & 0.69 & 1.25 & 2.33 & \textbf{0.57} & \textbf{1.02} & \textbf{2.07} \\
		remote		& 0.95 & 1.08 & 1.58 & 0.82 & 1.02 & 1.29 & 0.44 & 0.58 & 0.78 & 0.27 & 0.42 & 0.61 & \textbf{0.23} & \textbf{0.35} & \textbf{0.49} \\
		rocket		& 1.39 & 1.22 & 2.01 & 0.97 & 0.79 & 1.60 & 0.39 & 0.72 & 1.39 & 0.28 & 0.51 & 1.02 & \textbf{0.25} & \textbf{0.50} & \textbf{0.93} \\
		skateboard	& 1.97 & 1.78 & 2.45 & 0.93 & 1.07 & 1.83 & 0.52 & 0.80 & 1.31 & 0.35 & 0.56 & 0.92 & \textbf{0.24} & \textbf{0.43} & \textbf{0.77} \\
		tower		& 2.37 & 2.40 & 4.35 & 1.35 & 1.80 & 3.85 & 0.82 & 1.35 & 2.48 & 0.51 & 0.92 & 1.87 & \textbf{0.42} & \textbf{0.81} & \textbf{1.70} \\
		washer		& 2.77 & 2.52 & 4.64 & 1.83 & 1.97 & 5.28 & 1.04 & 1.39 & 2.73 & 0.61 & 0.87 & 1.94 & \textbf{0.53} & \textbf{0.73} & \textbf{1.59} \\
		\midrule[0.3pt]
		mean		& 3.22 & 3.13 & 5.43 & 1.84 & 2.23 & 4.95 & 1.05 & 1.67 & 3.45 & 0.61 & 1.07 & 2.35 & \textbf{0.55} & \textbf{0.99} & \textbf{2.15} \\
		\bottomrule[1pt]
	\end{tabular}
	}
	\label{table:result-sp21-complete}
\end{table*}

==> tables/result-sp55-complete.tex <==
% shapenet55 more
\begin{table*}[t]
	\centering
	% \small
    % \footnotesize
    % \normalsize
	% \scriptsize
	% \setlength{\tabcolsep}{4.5pt}
	\setlength{\arrayrulewidth}{0.7pt}
	\caption{Detailed results on ShapeNet-55 dataset. $S.$, $M.$ and $H.$ stand for the simple, moderate and hard difficulty levels.}
	\resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
		\toprule[1pt]
		 & \multicolumn{3}{c|}{PCN~\cite{yuan2018pcn}} & \multicolumn{3}{c|}{GRNet~\cite{xie2020grnet}} & \multicolumn{3}{c|}{PoinTr~\cite{yu2021pointr}} & \multicolumn{3}{c|}{SeedFormer~\cite{zhou2022seedformer}} &
         \multicolumn{3}{c}{Ours}\\
				& S. & M. & H. & S. & M. & H. & S. & M. & H. & S. & M. & H. & S. & M. & H. \\
		\midrule[0.3pt]
		airplane 	   & 0.90 & 0.89 & 1.32 & 0.87 & 0.87 & 1.27 & 0.27 & 0.38 & 0.69 & 0.23 & 0.35 & 0.61 & \textbf{0.20} & \textbf{0.30} & \textbf{0.51} \\
        trash-bin 	   & 2.16 & 2.18 & 5.15 & 1.69 & 2.01 & 3.48 & 0.80 & 1.15 & 2.15 & 0.73 & 1.08 & 1.94 & \textbf{0.59} & \textbf{0.85} & \textbf{1.48} \\
        bag 		   & 2.11 & 2.04 & 4.44 & 1.41 & 1.70 & 2.97 & 0.53 & 0.74 & 1.51 & 0.43 & 0.67 & 1.28 & \textbf{0.35} & \textbf{0.55} & \textbf{1.06} \\
        basket 		   & 2.21 & 2.10 & 4.55 & 1.65 & 1.84 & 3.15 & 0.73 & 0.88 & 1.82 & 0.65 & 0.83 & 1.54 & \textbf{0.59} & \textbf{0.72} & \textbf{1.35} \\
        bathtub 	   & 2.11 & 2.09 & 3.94 & 1.46 & 1.73 & 2.73 & 0.64 & 0.94 & 1.68 & 0.52 & 0.82 & 1.45 & \textbf{0.44} & \textbf{0.67} & \textbf{1.16} \\
        bed 		   & 2.86 & 3.07 & 5.54 & 1.64 & 2.03 & 3.70 & 0.76 & 1.10 & 2.26 & 0.63 & 0.91 & 1.89 & \textbf{0.51} & \textbf{0.78} & \textbf{1.63} \\
        bench 		   & 1.31 & 1.24 & 2.14 & 1.03 & 1.09 & 1.71 & 0.38 & 0.52 & 0.94 & 0.32 & 0.42 & 0.84 & \textbf{0.26} & \textbf{0.33} & \textbf{0.61} \\
        birdhouse 	   & 3.29 & 3.53 & 6.69 & 1.87 & 2.40 & 4.71 & 0.98 & 1.49 & 3.13 & 0.76 & 1.30 & 2.46 & \textbf{0.67} & \textbf{1.11} & \textbf{2.11} \\
        bookshelf 	   & 2.70 & 2.70 & 4.61 & 1.42 & 1.71 & 2.78 & 0.71 & 1.06 & 1.93 & 0.57 & 0.84 & 1.57 & \textbf{0.51} & \textbf{0.74} & \textbf{1.33} \\
        bottle 		   & 1.25 & 1.43 & 4.61 & 1.05 & 1.44 & 2.67 & 0.37 & 0.74 & 1.50 & 0.31 & 0.63 & 1.21 & \textbf{0.26} & \textbf{0.53} & \textbf{1.02} \\
        bowl 		   & 2.05 & 1.83 & 3.66 & 1.60 & 1.77 & 2.99 & 0.68 & 0.78 & 1.44 & 0.56 & 0.65 & 1.18 & \textbf{0.46} & \textbf{0.51} & \textbf{0.86} \\
        bus 		   & 1.20 & 1.14 & 2.08 & 1.06 & 1.16 & 1.48 & 0.42 & 0.55 & 0.79 & 0.42 & 0.55 & 0.73 & \textbf{0.34} & \textbf{0.45} & \textbf{0.60} \\
        cabinet 	   & 1.60 & 1.49 & 3.47 & 1.27 & 1.41 & 2.09 & 0.55 & 0.66 & 1.16 & 0.57 & 0.69 & 1.05 & \textbf{0.47} & \textbf{0.54} & \textbf{0.83} \\
        camera 		   & 4.05 & 4.54 & 8.27 & 2.14 & 3.15 & 6.09 & 1.10 & 2.03 & 4.34 & 0.83 & 1.68 & 3.45 & \textbf{0.68} & \textbf{1.39} & \textbf{2.82} \\
        can 		   & 2.02 & 2.28 & 6.48 & 1.58 & 2.11 & 3.81 & 0.68 & 1.19 & 2.14 & 0.58 & 1.03 & 1.79 & \textbf{0.49} & \textbf{0.84} & \textbf{1.50} \\
        cap 		   & 1.82 & 1.76 & 4.20 & 1.17 & 1.37 & 3.05 & 0.46 & 0.62 & 1.64 & 0.33 & 0.45 & 1.18 & \textbf{0.28} & \textbf{0.36} & \textbf{0.64} \\
        car 		   & 1.48 & 1.47 & 2.60 & 1.29 & 1.48 & 2.14 & 0.64 & 0.86 & 1.25 & 0.65 & 0.86 & 1.17 & \textbf{0.48} & \textbf{0.67} & \textbf{0.92} \\
        cellphone 	   & 0.80 & 0.79 & 1.71 & 0.82 & 0.91 & 1.18 & 0.32 & 0.39 & 0.60 & 0.31 & 0.40 & 0.54 & \textbf{0.26} & \textbf{0.31} & \textbf{0.40} \\
        chair 		   & 1.70 & 1.81 & 3.34 & 1.24 & 1.56 & 2.73 & 0.49 & 0.74 & 1.63 & 0.41 & 0.65 & 1.38 & \textbf{0.32} & \textbf{0.51} & \textbf{1.10} \\
        clock 		   & 2.10 & 2.01 & 3.98 & 1.46 & 1.66 & 2.67 & 0.62 & 0.84 & 1.65 & 0.53 & 0.74 & 1.35 & \textbf{0.43} & \textbf{0.61} & \textbf{1.10} \\
        keyboard 	   & 0.82 & 0.82 & 1.04 & 0.74 & 0.81 & 1.09 & 0.30 & 0.39 & 0.45 & 0.28 & 0.36 & 0.45 & \textbf{0.23} & \textbf{0.27} & \textbf{0.33} \\
        dishwasher 	   & 1.93 & 1.66 & 4.39 & 1.43 & 1.59 & 2.53 & 0.55 & 0.69 & 1.42 & 0.56 & 0.69 & 1.30 & \textbf{0.48} & \textbf{0.55} & \textbf{1.07} \\
        display 	   & 1.56 & 1.66 & 3.26 & 1.13 & 1.38 & 2.29 & 0.48 & 0.67 & 1.33 & 0.39 & 0.59 & 1.10 & \textbf{0.33} & \textbf{0.47} & \textbf{0.89} \\
        earphone 	   & 3.13 & 2.94 & 7.56 & 1.78 & 2.18 & 5.33 & 0.81 & 1.38 & 3.78 & 0.64 & 1.04 & \textbf{2.75} & \textbf{0.52} & \textbf{0.79} & 3.05 \\
        faucet 		   & 3.21 & 3.48 & 7.52 & 1.81 & 2.32 & 4.91 & 0.71 & 1.42 & 3.49 & 0.55 & 1.15 & 2.63 & \textbf{0.52} & \textbf{1.03} & \textbf{2.26} \\
        filecabinet    & 2.02 & 1.97 & 4.14 & 1.46 & 1.71 & 2.89 & 0.63 & 0.84 & 1.69 & 0.63 & 0.84 & 1.49 & \textbf{0.55} & \textbf{0.71} & \textbf{1.27} \\
        guitar 		   & 0.42 & 0.38 & 1.23 & 0.44 & 0.48 & 0.76 & 0.14 & 0.21 & 0.42 & 0.13 & 0.19 & 0.32 & \textbf{0.10} & \textbf{0.17} & \textbf{0.28} \\
        helmet 		   & 3.76 & 4.18 & 7.53 & 2.33 & 3.18 & 6.03 & 0.99 & 1.93 & 4.22 & 0.79 & 1.52 & 3.61 & \textbf{0.62} & \textbf{1.18} & \textbf{3.09} \\
        jar 		   & 2.57 & 2.82 & 6.00 & 1.72 & 2.37 & 4.37 & 0.77 & 1.33 & 2.87 & 0.63 & 1.13 & 2.36 & \textbf{0.52} & \textbf{0.90} & \textbf{1.96} \\
        knife 		   & 0.94 & 0.62 & 1.37 & 0.72 & 0.66 & 0.96 & 0.20 & 0.33 & 0.56 & 0.15 & 0.28 & 0.45 & \textbf{0.14} & \textbf{0.24} & \textbf{0.40} \\
        lamp 		   & 3.10 & 3.45 & 7.02 & 1.68 & 2.43 & 5.17 & 0.64 & 1.40 & 3.58 & 0.45 & 1.06 & \textbf{2.67} & \textbf{0.44} & \textbf{1.05} & \textbf{2.67} \\
        laptop 		   & 0.75 & 0.79 & 1.59 & 0.83 & 0.87 & 1.28 & 0.32 & 0.34 & 0.60 & 0.32 & 0.37 & 0.55 & \textbf{0.27} & \textbf{0.28} & \textbf{0.41} \\
        loudspeaker    & 2.50 & 2.45 & 5.08 & 1.75 & 2.08 & 3.45 & 0.78 & 1.16 & 2.17 & 0.67 & 1.01 & 1.80 & \textbf{0.54} & \textbf{0.82} & \textbf{1.54} \\
        mailbox 	   & 1.66 & 1.74 & 5.18 & 1.15 & 1.59 & 3.42 & 0.39 & 0.78 & 2.56 & 0.30 & 0.67 & 2.04 & \textbf{0.25} & \textbf{0.57} & \textbf{1.49} \\
        microphone 	   & 3.44 & 3.90 & 8.52 & 2.09 & 2.76 & 5.70 & 0.70 & 1.66 & 4.48 & 0.62 & \textbf{1.61} & 3.66 & \textbf{0.60} & 1.76 & \textbf{3.52} \\
        microwaves 	   & 2.20 & 2.01 & 4.65 & 1.51 & 1.72 & 2.76 & 0.67 & 0.83 & 1.82 & 0.63 & 0.79 & 1.47 & \textbf{0.54} & \textbf{0.65} & \textbf{1.24} \\
        motorbike 	   & 2.03 & 2.01 & 3.13 & 1.38 & 1.52 & 2.26 & 0.75 & 1.10 & 1.92 & 0.68 & 0.96 & 1.44 & \textbf{0.51} & \textbf{0.78} & \textbf{1.22} \\
        mug 		   & 2.45 & 2.48 & 5.17 & 1.75 & 2.16 & 3.79 & 0.91 & 1.17 & 2.35 & 0.79 & 1.03 & 2.06 & \textbf{0.64} & \textbf{0.88} & \textbf{1.67} \\
        piano 		   & 2.64 & 2.74 & 4.83 & 1.53 & 1.82 & 3.21 & 0.76 & 1.06 & 2.23 & 0.62 & 0.87 & 1.79 & \textbf{0.48} & \textbf{0.65} & \textbf{1.31} \\
        pillow 		   & 1.85 & 1.81 & 3.68 & 1.42 & 1.67 & 3.04 & 0.61 & 0.82 & 1.56 & 0.48 & 0.75 & 1.41 & \textbf{0.37} & \textbf{0.50} & \textbf{0.93} \\
        pistol 		   & 1.25 & 1.17 & 2.65 & 1.11 & 1.06 & 1.76 & 0.43 & 0.66 & 1.30 & 0.37 & 0.56 & 0.96 & \textbf{0.31} & \textbf{0.50} & \textbf{0.81} \\
        flowerpot 	   & 3.32 & 3.39 & 6.04 & 2.02 & 2.48 & 4.19 & 1.01 & 1.51 & 2.77 & 0.93 & 1.30 & 2.32 & \textbf{0.72} & \textbf{1.07} & \textbf{1.96} \\
        printer 	   & 2.90 & 3.19 & 5.84 & 1.56 & 2.38 & 4.24 & 0.73 & 1.21 & 2.47 & 0.58 & 1.11 & 2.13 & \textbf{0.50} & \textbf{0.86} & \textbf{1.79} \\
        remote 		   & 0.99 & 0.97 & 2.04 & 0.89 & 1.05 & 1.29 & 0.36 & 0.53 & 0.71 & 0.29 & 0.46 & 0.62 & \textbf{0.23} & \textbf{0.38} & \textbf{0.48} \\
        rifle 		   & 0.98 & 0.80 & 1.31 & 0.83 & 0.77 & 1.16 & 0.30 & 0.45 & 0.79 & 0.27 & 0.41 & 0.66 & \textbf{0.22} & \textbf{0.35} & \textbf{0.57} \\
        rocket 		   & 1.05 & 1.04 & 1.87 & 0.78 & 0.92 & 1.44 & 0.23 & 0.48 & 0.99 & 0.21 & 0.46 & 0.83 & \textbf{0.15} & \textbf{0.36} & \textbf{0.73} \\
        skateboard 	   & 1.04 & 0.94 & 1.68 & 0.82 & 0.87 & 1.24 & 0.28 & 0.38 & 0.62 & 0.23 & 0.32 & 0.62 & \textbf{0.18} & \textbf{0.27} & \textbf{0.41} \\
        sofa 		   & 1.65 & 1.61 & 2.92 & 1.35 & 1.45 & 2.32 & 0.56 & 0.67 & 1.14 & 0.50 & 0.62 & 1.02 & \textbf{0.41} & \textbf{0.49} & \textbf{0.79} \\
        stove 		   & 2.07 & 2.02 & 4.72 & 1.46 & 1.72 & 3.22 & 0.63 & 0.92 & 1.73 & 0.59 & 0.87 & 1.49 & \textbf{0.51} & \textbf{0.74} & \textbf{1.24} \\
        table 		   & 1.56 & 1.50 & 3.36 & 1.15 & 1.33 & 2.33 & 0.46 & 0.64 & 1.31 & 0.41 & 0.58 & 1.18 & \textbf{0.35} & \textbf{0.47} & \textbf{0.91} \\
        telephone 	   & 0.80 & 0.80 & 1.67 & 0.81 & 0.89 & 1.18 & 0.31 & 0.38 & 0.59 & 0.31 & 0.39 & 0.55 & \textbf{0.26} & \textbf{0.31} & \textbf{0.43} \\
        tower 		   & 1.91 & 1.97 & 4.47 & 1.26 & 1.69 & 3.06 & 0.55 & 0.90 & 1.95 & 0.47 & 0.84 & 1.65 & \textbf{0.40} & \textbf{0.72} & \textbf{1.56} \\
        train 		   & 1.50 & 1.41 & 2.37 & 1.09 & 1.14 & 1.61 & 0.50 & 0.70 & 1.12 & 0.51 & 0.66 & 1.01 & \textbf{0.37} & \textbf{0.53} & \textbf{0.82} \\
        watercraft 	   & 1.46 & 1.39 & 2.40 & 1.09 & 1.12 & 1.65 & 0.41 & 0.62 & 1.07 & 0.35 & 0.56 & 0.92 & \textbf{0.28} & \textbf{0.48} & \textbf{0.79} \\
        washer 		   & 2.42 & 2.31 & 6.08 & 1.72 & 2.05 & 4.19 & 0.75 & 1.06 & 2.44 & 0.64 & 0.91 & 2.04 & \textbf{0.56} & \textbf{0.74} & \textbf{1.51} \\
		\midrule[0.3pt]
		mean 		   & 1.96 & 1.98 & 4.09 & 1.35 & 1.63 & 2.86 & 0.58 & 0.88 & 1.80 & 0.50 & 0.77 & 1.49 & \textbf{0.41} & \textbf{0.64} & \textbf{1.25} \\
		\bottomrule[1pt]
	\end{tabular}
	}
	\label{table:result-sp55-complete}
\end{table*}
